Reflections on Designing and Running Visualization Design and Programming Activities in Courses with Many Students

In this paper, we reflect on the educational challenges and research opportunities in running data visualization design activities in the context of large courses. With the increasing number and sizes of data visualization course, we need to better understand approaches to scaling our teaching efforts. We draw on experiences organizing and facilitating activities primarily based on one instance of a master's course given to about 130 students. We provide a detailed account of the course with particular focus on the purpose, structure, and outcome of six two-hour design activities. Based on this, we reflect on three aspects of the course: First, how the course scale led us to thoroughly plan, evaluate, and revise communication between students, teaching assistants, and lecturers. Second, how we designed learning scaffolds through the design activities, and the reflections we received from students on this matter. Finally, we reflect on the diversity of the students that followed the course, the visualization exercises we used, the projects they worked on, and when to key in on simple boring problems and data sets. Thus, our paper contributes with discussions about balancing topical diversity, scaling courses to many students, and problem-based learning.

==> tables/altair-table-alt.tex <==
\begin{table*}[h!]
    \caption{Tasks for the four Altair exercise sessions. }
    \label{tab:altair-table-alt}
    \centering
	\setlength\tabcolsep{0.10cm}
	\def\arraystretch{0.99}
    % \small
    % \footnotesize
    \mycfs{7.3}
 \begin{tabularx}{\linewidth}{@{} p{.9cm} p{.9cm} p{.5cm} p{5.95cm} @{\hskip .45cm} p{.9cm} p{.9cm} p{.5cm} p{5.9cm} @{}}
    \hline
\\[-6pt]
\textbf{Exercise} & \textbf{Focus} & \textbf{Task} & \textbf{Title} &
\textbf{Exercise} & \textbf{Focus} & \textbf{Task} & \textbf{Title} \\
\\[-6pt]
    \hline
\\[-3pt]
    \multicolumn{4}{@{} l }{\textbf{Intro to Altair}} & 
    \multicolumn{4}{@{} l }{\textbf{Domains and scales}} \\
    % \cline{1-2}
\\[-6pt]
    A1 & Colab  & T1 & Install the Altair library &
    A2 & Colab  & T1 & Install the Altair library \\
       &        & T2 & Import pandas, numpy and altair &
       &        & T2 & How to connect to a shared folder \\
       & Pandas & T3 & Import the cereal .csv file into a DataFrame &
       &        & T3 & Import pandas and altair \\
       &        & T4 & Display a single column from a DataFrame &
       & Pandas & T4 & Import the cereal .csv file into a DataFrame \\
       &        & T5 & Rename a column &
       &        & T5 & Display the first five rows of a DataFrame \\
       &        & T6 & Find the product with the highest and the lowest rating &
       & Altair & T6 & Changing colors of chart \\
       & Altair & T7 & Create a scatterplot &
       &        & T7 & Create a scatterplot of \textit{sodium} and \textit{rating}, and make the color of the data points dependent on \textit{mfr} \\
       &        & T8 & Make the scatterplot interactive &
       &        & T8 & Change the colors of the data points in the chart \\
       &        & T9 & Create other data visualizations \\
       &        & T10 & Make the data visualization interactive \\
\\
    \multicolumn{4}{@{} l }{\textbf{Faceting and multiple views}} &
    \multicolumn{4}{@{} l }{\textbf{Specifying interaction}} \\
    % \cline{1-3}
\\[-6pt]
    A3 & Colab  & T1 & Install the Altair library &
    A4 & Colab  & T1 & Install the Altair library \\
       &        & T2 & Import pandas and altair &
       &        & T2 & Import pandas and altair \\
       & Pandas & T3 & Import the cereal .csv file into a DataFrame &
       & Pandas & T3 & Import the cereal .csv file into a DataFrame \\
       & Altair & T4 & Plotting two charts next to each other &
       & Altair & T4 & Interval selections \\
       &        & T5 & Layering two charts so one is on top of the other &
       &        & T5 & Multiple selections \\
       &        & T6 & Adding interaction between a bar chart and scatterplot &
       &        & T6 & Point selections \\
       &        &    &                  &
       &        & T7 & Tooltip channels \\
\\[-6pt]
    \hline
    \end{tabularx}
\end{table*}



==> tables/altair-table.tex <==
\begin{table}[b!]
    \caption{Tasks for the four Altair exercise sessions. }
    \label{tab:programming-exercises}
    \centering
	\setlength\tabcolsep{0.10cm}
	\def\arraystretch{0.99}
    % \small
    \footnotesize
 \begin{tabularx}{\linewidth}{@{} p{1.1cm} p{.9cm} p{.9cm} X @{}}
    \hline
\\[-6pt]
\textbf{Exercise} & \textbf{Focus} & \textbf{Task} & \textbf{Title} \\
\\[-6pt]
    \hline
\\[-3pt]
    \multicolumn{4}{@{} l }{\textbf{Intro to Altair}} \\
    % \cline{1-2}
\\[-6pt]
    A1 & Colab  & T1 & Install the Altair library \\
       &        & T2 & Import pandas, numpy and altair \\
       & Pandas & T3 & Import the cereal .csv file into a DataFrame \\
       &        & T4 & Display a single column from a DataFrame \\
       &        & T5 & Rename a column \\
       &        & T6 & Find the product with the highest and the lowest rating \\
       & Altair & T7 & Create a scatterplot \\
       &        & T8 & Make the scatterplot interactive \\
       &        & T9 & Create other data visualizations \\
       &        & T10 & Make the data visualization interactive \\
\\[-6pt]
    % \hline
\\[-3pt]
    \multicolumn{4}{@{} l }{\textbf{Domains and scales}} \\
    % \cline{1-2}
\\[-6pt]
    A2 & Colab  & T1 & Install the Altair library \\
       &        & T2 & How to connect to a shared folder \\
       &        & T3 & Import pandas and altair \\
       & Pandas & T4 & Import the cereal .csv file into a DataFrame \\
       &        & T5 & Display the first five rows of a DataFrame \\
       & Altair & T6 & Changing colors of chart \\
       &        & T7 & Create a scatterplot of \textit{sodium} and \textit{rating}, and make the color of the data points dependent on \textit{mfr} \\
       &        & T8 & Change the colors of the data points in the chart \\
\\[-6pt]
    % \hline
\\[-3pt]
    \multicolumn{4}{@{} l }{\textbf{Faceting and multiple views}} \\
    % \cline{1-3}
\\[-6pt]
    A3 & Colab  & T1 & Install the Altair library \\
       &        & T2 & Import pandas and altair \\
       & Pandas & T3 & Import the cereal .csv file into a DataFrame \\
       & Altair & T4 & Plotting two charts next to each other \\
       &        & T5 & Layering two charts so one is on top of the other \\
       &        & T6 & Adding interaction between the bar chart and the scatterplot\\
\\[-6pt]
    % \hline
\\[-3pt]
    \multicolumn{4}{@{} l }{\textbf{Specifying interaction}} \\
    % \cline{1-3}
\\[-6pt]
    A4 & Colab  & T1 & Install the Altair library \\
       &        & T2 & Import pandas and altair \\
       & Pandas & T3 & Import the cereal .csv file into a DataFrame \\
       & Altair & T4 & Interval selections \\
       &        & T5 & Multiple selections \\
       &        & T6 & Point selections \\
       &        & T7 & Tooltip channels \\
\\[-6pt]
    \hline
    \end{tabularx}
\end{table}



==> tables/programming-exercise-structure.tex <==
\begin{table*}[]
    \caption{Structure of programming exercises.}
    \label{tab:programming-exercise-structure}
    \centering
	\setlength\tabcolsep{0.10cm}
	\def\arraystretch{0.99}
    \small
 \begin{tabularx}{\linewidth}{@{} l l l @{}}
    \hline
\\[-6pt]
    \textbf{Week} & 
            \textbf{Date} & 
                    \textbf{Duration} & 
                                \textbf{Exercise} & 
                                            \textbf{Title} & 
                                                                                        \textbf{Reflections} &
                                                      \textbf{Literature} 
                                                                        \\
\\[-6pt]
    \hline
\\[-6pt]                                                                               
    1  &    Feb 10 & \\
\\[-6pt]
    \hline
\\[-6pt]
    2  &    Feb 17 & 105 minutes &  D1 &    Critique and redesign                       & 110\\
    3  &    Feb 24 &  45 minutes &  D2 &    Data collection and sketching               & 110 \\
    4  &    Mar  3 & 105 minutes &  D3 &    Constructive visualization                  & 90 \\
    5  &    Mar 10 & 105 minutes &  D4 &    Sketching and refining visualization ideas  & 50 \\
    6  &    Mar 17 & 105 minutes &  D5 &    Sketching in the digital medium             & 15 \\
\\[-6pt]
    \hline
\\[-6pt]
    7  &    Mar 24 & 105 minutes &  P1 &    Intro to Altair \\
    8  &    Mar 31 & 105 minutes &  P2 &    Domains and scales in Altair\\
    9  &    Apr 14 & 105 minutes &  P3 &    Faceting and multiple views in Altair \\
    10 &    Apr 21 & 105 minutes &  P4 &    Specifying interaction in Altair \\
\\[-6pt]
    \hline
\\[-6pt]
    11 &    Apr 28 & 105 minutes &  D6 &    Heuristic evaluation                        & 3 \\
\\[-6pt]
    \hline
\\[-6pt]
    12 &    May 12 &       &    \textit{Project work} \\
\\[-6pt]
    \hline
    \end{tabularx}
\end{table*}
